Probabilistic Fair Ordering of Events

A growing class of applications depends on fair ordering, where events that occur earlier should be processed before later ones. Providing such guarantees is difficult in practice because clock synchronization is inherently imperfect: events generated at different clients within a short time window may carry timestamps that cannot be reliably ordered. Rather than attempting to eliminate synchronization error, we embrace it and establish a probabilistically fair sequencing process. Tommy is a sequencer that uses a statistical model of per-clock synchronization error to compare noisy timestamps probabilistically. Although this enables ordering of two events, the probabilistic comparator is intransitive, making global ordering non-trivial. We address this challenge by mapping the sequencing problem to a classical ranking problem from social choice theory, which offers principled mechanisms for reasoning with intransitive comparisons. Using this formulation, Tommy produces a partial order of events, achieving significantly better fairness than a Spanner TrueTime-based baseline approach.

==> application-hedging.tex <==
\subsection{Application Hedging}
\label{sec:app-hedging}

In addition to unfairness caused by clock errors, \textbf{machine heterogeneity} can also significantly undermine fairness among clients. Prior work~\cite{vig-thesis} has shown that performance heterogeneity is common in cloud VMs: even instances of the same VM type can exhibit non-negligible performance differences.


Consider two clients that invoke a clock API on their local machines at the same true time. Ideally, both clients should receive timestamps simultaneously and thus have equal opportunity when competing for shared resources. In practice, however, the latency incurred within the machine’s software stack varies across VMs. A client running on a less performant machine is therefore more likely to receive a later timestamp, placing it at a systematic disadvantage. Over time, such bias accumulates and leads to persistent unfairness.


To mitigate this issue, we propose \textbf{application hedging}. Instead of permanently pinning each client application to a fixed machine, we periodically rotate client applications across machines at runtime. This rotation ensures that no client consistently benefits from, or is penalized by, the performance characteristics of a particular machine.


We evaluate the effectiveness of application hedging using two groups of simulations. In each group, we simulate 10 clients that invoke the clock API simultaneously. To model heterogeneity, we inject artificial latency between the API invocation and the receipt of the returned timestamp. Each machine is assigned a distinct latency distribution. In the first group (Figure~\ref{fig:app_hedging_case_1}), machine~$i$ is assigned an injected latency $L_i \sim \mathcal{N}(i, 10)$~\si{\micro\second}. In the second group
(Figure~\ref{fig:app_hedging_case_2}), we use
$L_i \sim \mathcal{N}(i, 1)$. Although both groups share the same ordering
of mean latencies, the second group has a significantly smaller variance,
resulting in substantially less overlap among latency distributions.
Consequently, machine performance is \emph{more strongly ordered} and
heterogeneity is more pronounced: for $i < j$, machine~$i$ is much more
likely to return API results earlier than machine~$j$.



We rank clients based on the order in which they receive API responses. We repeat the experiment over multiple trials and compute the average rank for each client. In the absence of heterogeneity, all clients should achieve similar average ranks. However, when each client is fixed to a single machine, the average ranks exhibit substantial variance, reflecting persistent unfairness. In contrast, application hedging significantly reduces rank variance by distributing machine-induced advantages and disadvantages across clients.

This effect becomes even more pronounced in the high-heterogeneity setting (Figure~\ref{fig:app_hedging_case_2}), where application hedging yields a clear improvement in fairness. These results demonstrate that rotating client applications across machines is an effective mechanism for mitigating unfairness caused by machine heterogeneity.


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/app_hedging_case_1.png}
    \caption{Fairness (average rank) comparison running on machines with low heterogeneity}
    \label{fig:app_hedging_case_1}
\end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/app_hedging_case_2.png}
    \caption{Fairness (average rank) comparison running on machines with high heterogeneity}
    \label{fig:app_hedging_case_2}
\end{figure}
